Scheduling Task-parallel Applications in Dynamically Asymmetric Environments

Shared resource interference is observed by applications as dynamic performance asymmetry. Prior art has developed approaches to reduce the impact of performance asymmetry mainly at the operating system and architectural levels. In this work, we study how application-level scheduling techniques can leverage moldability (i.e. flexibility to work as either single-threaded or multithreaded task) and explicit knowledge on task criticality to handle scenarios in which system performance is not only unknown but also changing over time. Our proposed task scheduler dynamically learns the performance characteristics of the underlying platform and uses this knowledge to devise better schedules aware of dynamic performance asymmetry, hence reducing the impact of interference. Our evaluation shows that both criticality-aware scheduling and parallelism tuning are effective schemes to address interference in both shared and distributed memory applications

==> 1-abstract-new.tex <==
Modern computing platforms exhibit performance asymmetry. Among other factors, the performance of parallel applications on such platforms is often influenced by i) presence of big.LITTLE cores ii) cores operating on different frequencies iii) interference from co-running applications or the OS. Prior research has mainly focused on mitigating the effects of interference - e.g., through lightweight kernels and better job scheduling techniques - or by better adapting to asymmetry - through scheduling techniques that are aware of the underlying hardware performance asymmetry. However, in real systems the varied sources of performance asymmetry often co-exist.

%These solutions however have limited effectiveness for parallel applications since are not effective at tackling the varying sources of asymmetry which often coexists in a real system .

We propose a scheduling technique for parallel applications which can adapt to varied sources of asymmetry dynamically during execution. 
%We propose a novel scheduler that dynamically learns and adapts to asym-metric architectures and dynamically determines the best task schedules in the presence of interference. 
The scheduler uses history of task execution times computed on different cores to build a Performance Trace Table (PTT) that enables it to learn and react to asymmetry. The PTT enables the scheduler to specifically guide both the selection of core that should execute a task and the resource container (numer of cores) allocated for each task to best mitigate the effects of asymmetry. We evaluate the proposed scheduler using microbechmarks and real application on an NVIDIA Jetson TX2 system featuring asymmetric CPU clusters and on a dual-socket 10-core Intel Haswell system. Our evaluation shows that, in the presence of interference and architecture asymmetry, the proposed scheduling technique outperforms both random work stealing as well as state-of-the-art criticality-aware technique based on a fixed notion of hardware performance asymmetry.

==> 1-abstract.tex <==
\begin{abstract}
The performance of parallel applications can be severely impacted in the presence of interference, be it due to co-scheduling of applications, OS noise (aka jitter) or DVFS activity due to power management governors. % or other causes. 
%Moreoever, in modern computing systems, performance asymmetry introduced due to DVFS, diverse cores and memory hierarchies has been shown to further exacerbate the detrimental impact of interference. 
Prior research has mainly focused on mitigating the effects of interference by developing lightweight OS kernels and attempting to isolate applications by reducing shared resources. %introducing job-scheduling techniques for non-destructive co-scheduling. % need to collect vast amount of references
However, unpredictable events such as job arrivals or DVFS for power capping, means that interference is bound to happen. As system size and users increase, so does interference. 
%	power dynamics in modern data centers translate into unpredictable DVFS activity which reduces the usefulness of such techniques.
This leads to the question of how an application should react when interference finally occurs.

Unlike prior art, we study runtime techniques to detect and schedule around interference.
%	to address variability via a novel scheduler that dynamically learns and adapts to episodes of interference. 
%ing technique for mixed mode DAG-based parallel applications. 
In this paper we propose a task-parallel scheduler that uses history of task execution times computed on different core partitions to build a performance model that enables it to learn and react to interference. 
It does so by guiding both the selection of execution threads and of the resource container allocated for each task. 
We evaluate the proposed scheduler using both synthetic workloads and benchmarks including K-means, Breadth-First Search and the Darknet-VGG-16 image classification framework %based on Convolutional Neural Networks (CNN) 
on an NVIDIA Jetson TX2 board featuring asymmetric CPU clusters and on a homogeneous dual-socket 10-core Intel Haswell system. 
Our evaluation shows that the proposed schemes offer better robustness against scheduling schemes implemented in modern runtimes, such as work stealing or OpenMP loop schedulers. % such as OpenMP or Cilk.% both random work stealing as well as scheduling schemes that consider static interference. 
% miquelp: I am not sure we should talk about FAS in the abstract since it's goal is not clear at this point. In fact, I am even wondering if FAS should be evaluated at all, or we should just stick to work stealing and openmp which is what people use in practice...
%	based on a fixed notion of hardware performance asymmetry.
Our schemes are orthogonal to lightweight kernels and job scheduling approaches and can thus be used in combination with these. % Although this is not evaluated, it seems obvious enough to state.
% remove criticality-awareness since at this point it is not clear how they help in interference awareness
%, but also reduces the performance impact suffered by the interfering application.  -- this is not shown

% miquelp: so I added the above paragraph because we need to somehow set the context. The below text sounds to me more like classical scheduling paper, which is what we want to avoid so that we do not get the same type of comments as ICPP.
%Madhavan: Performance asymmetry is an inherent aspect of modern computing systems. Such asymmetry can typically be attributed to the core or the memory system characteristics (big/LITTLE cores, DVFS, NUCA/NUMA effects etc.) or to the changes introduced in the execution environment (OS interference, application interference etc.). Prior research has mostly focused on addressing scheduling challenges on such asymmetric systems at the OS-level. In contrast, this paper proposes an application-level scheduling strategy for parallel mixed-mode DAGs, which are considered to be a promising execution model for modern asymmetric systems. The proposed adaptive online scheduler uses history of task execution times computed on different cores to build a Performance Trace Table (PTT),and in turn guide the scheduling of tasks and  determine how much execution resources must be assigned to each. ADD SUMMARY OF RESULTS. Our evaluation shows that the proposed approach, although simple, is effective at recognizing the performance asymmetry in the system and guide scheduling of high and low priority tasks to suitable cores and assign the appropriate amount of resources.
% Specifically, we propose an adaptive online scheduler based on Performance Trace Table (PTT), which is an extensible and dynamic lightweight manifest of the per-core latency that can be used to guide the scheduling of both high and low priority tasks. By understanding carefully chosen online performance parameters, the PTT decides the elasticity and moldablity of tasks to maximize performance in the presence of static and dynamic performance asymmetry as well as inter-application interference. We benchmark a synthetic Direct Acyclic Graph (DAG) of different workload categories on NVIDIA Jetson TX2 chip featuring asymmetric CPU clusters. {\color{red} Our runs achieve ...}. The dynamic interference analysis addresses OS-level interference due to frequency scaling that results from realistic Governor policies on a quad-socket 12-core AMD Opteron\texttrademark\/Processor 6348. The proposed scheduler maintains a consistent advantage over {\color{red} the work-stealing scheduler?} by minimizing the effect of frequency scaling on high-priority tasks. Inter-application interference on both compute and memory resources is also studied in light of a ported implementation of the Darknet-VGG-16 image classification framework based on Convolutional Neural Networks (CNN).  {\color{red} We show that ...}
\end{abstract}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Modern computing platforms exhibit performance asymmetry. The performance of parallel applications on such platforms is influenced by different sources of asymmetry -  presence of big.LITTLE cores (A), interference from co-running applications or the OS  (B) etc. Prior research has mainly focused on mitigating the effects of interference by developing lightweight kernels and introducing job scheduling techniques for non-destructive co-scheduling or by proposing scheduling techniques that can adapt to asymmetric architectures without focusing on interference. These solutions however have limited effectiveness for parallel applications since are not effective at tackling the varying sources of asymmetry.
% no solution for parallel applications that targets both A and B, and C... D....

% We propose a novel scheduler that dynamically learns and adapts to asymmetric architectures and dynamically determines the best task schedules in the presence of interference. The proposed scheduler uses history of task execution times computed on different cores to build a Performance Trace Table (PTT) that enables it to learn and react to interference and asymmetry. It does so by guiding both the selection of execution threads and of the resource container allocated for each task. We evaluate the proposed scheduler using both synthetic workloads and the Darknet-VGG-16 image classification framework on an NVIDIA Jetson TX2 chip featuring asymmetric CPU clusters and on a dual-socket 10-core Intel Haswell system. Our evaluation shows that, in the presence of interfer-
% ence, the proposed PTT-based schemes outperform both random work stealing as well as state-of-the-art criticality-aware schemes based on a fixed notion of hardware performance asymmetry.


% story:
% 1. motivate interference and why it is important
%  1) co-scheduling of processes
%  2) OS jitter, daemon execution
%  3) DVFS activity to address power capping
%  4) intra-application contention?
%  5) types of interference: overlapping and non-overlapping
%  -> sources of dynamic asymmetry
% 2. what has been done to address interference (cite this one https://dl.acm.org/citation.cfm?id=3337907)
% 2.1 removing OS noise sources (lightweight kernels), 
% 2.2 isolation (caching, scheduling), ...
% 3. But what can the application do to avoid interference?
% 4. State problem statement and scope:
%    4.1 Scope: Parallel Workloads composed of tasks.
%    4.2 Scope: interference consists of overlapping and non-overlapping interference
%    4.3 Scope: performance-symmetric and performance-asymmetric multicores
%    PS: how to design a scheduler that learns and adapts to interference
% 5. In this paper we propose....
% 6. We explore the impact of task moldability in this context...
% 7. The contributions are...
% motivation for lower degrees of parallelism: https://web.eecs.umich.edu/~subh/papers/parallelism-ISPASS-2019.pdf
% -> this furthermore motivates co-scheduling


==> 2-intro-new.tex <==
\section{Introduction}
Performance asymmetry is an inherent aspect of modern computing systems~\cite{sbala-isca05}. 
Asymmetry can be broadly attributed to two sources - static and dynamic. Static sources are fixed at design time (e.g., single-ISA cores with different compute capabilities like ARM's big.LITTLE architecture). Dynamic sources are due to changes in resource allocated to an application at runtime (e.g., DVFS~\cite{lesueur-hotpower10}, caches~\cite{iyer-sigmetrics07}). The allocation of shared resources (like LLC, memory bandwidth etc.)  can be severely impacted due to interference – be it from co-running applications~\cite{chiang-2011-interference_vms} or the OS~\cite{hoefler-sc10,ates-icpp19,skinner-wcs05}. Adapting to varying sources of performance asymmetry is critical to achieve efficient execution, especially for parallel applications in which inter-process synchronization can be frequent. Furthermore, the growing landscape of asymmetric system configurations complicates application scheduling since ensuring high, sustained and portable performance in such an environment is challenging. 

Task-based parallel programming models are a natural fit in this context because they allow for tasks to be scheduled dynamically based on resource availability. Modern programming models even accommodate features like inter-task dependency specification, task priority, intra-task parallelism to help improve parallelism exploitation [ref]. Although dynamic scheduling - based on work stealing - is widely used by many task-based runtime systems~\cite{contreras-iiswc11,duran-ppl11,frigo-cilk5} and is better suited at adapting to asymmetry than the static scheduling counterparts there is lot of scope for improvement. This is because the underlying greedy scheduling~\cite{blumofe-jacm99} technique  always attempts to schedule a ready task as long as there are idle processing units. This is irrespective of whether the resulting schedule may cause interference or without being aware of the performance capabilities of the underlying architecture which in-turn can result in performance deterioration. The problem is magnified by the bandwidth-constrained and cache-constrained nature of modern computing systems. 

Recent works have attempted to improve the performance of such models by exploiting information about static performance asymmetry to efficiently schedule tasks in an asymmetric architecture~\cite{cata}. They specifically leverage information about task priorities and schedule tasks with higher priorities on the large core in a big.LITTLE platform. Some works have attempted to study and address interference from the OS and co-running applications especially in the context of supercomputers, where application scalability is particularly impacted~\cite{hoefler-sc10}. Common strategies to reduce noise in this particular scenario include eliminating unnecessary activities such as process scheduling or memory management~\cite{moreira-sc06} and carefully managing interrupts to minimize application perturbation~\cite{riesen-cc09}. However, to our knowledge there are no proposed solutions in literature to address the diverse list of interference sources shown in Figure 1 since optimizing a system to eliminate all sources of interference is a challenging endeavor. Moreover, since varied sources of asymmetry often coexist in a real system, it is important to handle them effectively to mitigate the ill effects of performance asymmetry.

Our proposed approach adopts the view that asymmetry is likely to be present (even if some of the sources can be eliminated/mitigated), and instead tries to adapt software runtimes to deal with its effects. To this end, we take a priority-aware task scheduler using a fixed notion of performance asymmetry and extend it with a performance trace table (PTT) that reflects the system’s performance characteristics at runtime. Despite its simplicity, the PTT
provides enough information to enable the scheduler to become aware of asymmetry and then sc at runtime with minimum cost. Most notably, these benefits are achieved with no static knowledge about the features of the application, the interference in the system, nor the platform’s system topology. This guarantees that the approach is portable across systems.


In summary, this paper proposes a novel scheduling technique for parallel DAGs that provides the following features:
– Elasticity and moldability, such that it infers placement and resource
container width to maximize throughput for different workload categories.
– Asymmetry-awareness, such that it reacts to static and dynamic perfor-
mance asymmetry and discovers effective mappings of tasks to cores without
prior knowledge of the platform and the workload.
– Interference-awareness, which is achieved by seamlessly reducing the im-
pact of interference arising during execution.

The remainder of this paper is organized as follows. Section 2 describes the
assumptions on the execution environment that form the basis for this research.
We present our runtime approach in Section 3. Section 4 describes the experimen-
tal setup and benchmarks in detail, which are used to evaluate our approach in
Section 5. Section 6 describes related work, while Section 7 concludes the work.

==> 2-intro.tex <==
\section{Introduction}
Performance asymmetry is an inherent aspect of modern computing systems~\cite{sbala-isca05}. 
Sources of asymmetry can be broadly categorized into static and dynamic. Static sources are fixed at design time, for example, single-ISA cores with different compute capabilities (e.g.,~big.LITTLE), or asymmetric ISA systems consisting of processor cores and accelerators (e.g.,~CPU/GPU/FPGA platforms). Dynamic sources of asymmetry arise from runtime reconfiguration. The usage of Dynamic Voltage and Frequency Scaling (DVFS)~\cite{lesueur-hotpower10} to tune the performance and efficiency of individual cores or clusters of cores is a classical example of dynamic asymmetry. Another example is the usage of cache partitioning to tune cores to the working sets of applications~\cite{iyer-sigmetrics07}.

%To make matters worse, some dynamic sources of asymmetry are uncontrolled. %\textit{interference}. 
%Interference is another source of 
Nonetheless, dynamic asymmetry can also
%that leads to performance degradation 
result from \textit{interference} on shared resources. Interference refers to a change in the availability of a shared resource. It can occur within a process, e.g.,~ resulting from oversubscription of caches, processors and memory bandwidth, and across processes, e.g.,~resulting from the time-sharing of a single processing unit in order to run multiple concurrent applications or from co-scheduling several applications on a single node. Adapting to 
%such sources of 
performance asymmetry is critical to achieve efficient execution, especially for parallel applications in which inter-process synchronization is frequent. 
%Obviously, designing scheduling strategies that address all these sources of heterogeneity under a optimization target (performance, energy, etc.) is a complex task. 
Furthermore, the growing landscape of asymmetric system configurations complicates scheduling and performance portability. 
Designing a runtime strategy that address all these sources of asymmetry 
%under a optimization target (performance, energy, etc.) 
while delivering high and sustained performance is a challenging task. 

Earlier works have attempted to study and address interference. Characterization of interference in the context of supercomputers, where application scalability is particularly impacted, has been an active topic of research~\cite{hoefler-sc10,ates-icpp19,skinner-wcs05}. 
%Lightweight OS kernels remove unnecessary features that create jitter, such as interrupts. 
Common strategies to reduce noise in this particular scenario include eliminating unnecessary activities such as process scheduling or memory management~\cite{moreira-sc06} and carefully managing interrupts to minimize application perturbation~\cite{riesen-cc09}.
%the interrupts generated by the scheduler in an attempt to achieve jitter-free coordinated thread execution. 
In the data-center environment, reducing interference across virtual machines has been achieved by predicting interference and scheduling jobs in an interference-aware way~\cite{chiang-2011-interference_vms}. Unfortunately, such works address interference only in specialized environments, and cannot be easily adopted in other settings. 
Furthermore, considering the long and diverse list of interference sources shown in Figure~\ref{fig:is}, optimizing a system to eliminate all sources of interference is 
an unrealistic endeavor.
%often a challenging and unsuccessful endeavor. %is a hopeless endeavor. 

\begin{figure}[t]
    \centering
    \includegraphics[width=.65\columnwidth]{Figure/interference_sources.pdf}
    \caption{A (non-exhaustive) categorization of interference sources in parallel systems}
    \label{fig:is}
\end{figure}


%A scheduling solution for multi-threaded computations requires an overlying execution model that is flexible and effective while enabling performance portability.
%In this DAG, individual nodes are non-preemptive pieces of work and edges indicate dependencies (i.e.~happens-before) relations. 
%This model extends the classical single-threaded task-DAG model, in which each task can only be mapped to a single processor. 
%
%An important result from our research~\cite{pericas-taco18} is that 
Instead, we believe that a more fruitful approach is to accept that interference will be present, and try to adapt software runtimes to deal with its effects.
Unfortunately, modern software runtimes often rely on classical schedulers that were developed at a time when interference was not a major concern. As a consequence they are not well equipped to deal with it.
Greedy scheduling~\cite{blumofe-jacm99}, a scheme implemented by many runtime systems~\cite{contreras-iiswc11,duran-ppl11,frigo-cilk5}, 
%-a classic result in scheduling theory which states that, in the presence of abundant parallelism, keeping processors busy whenever there are ready tasks will result in linear speed-up~\cite{blumofe-jacm99} -- 
%often leads to resource oversubscription which causes intra-application interference. 
%\footnote{\url{https://www.karlrupp.net/2013/06/cpu-gpu-and-mic-hardware-characteristics-over-time/}}. 
%Greedy schedulers will 
always attempts to schedule a ready task as long as there are idle processing units, even if the resulting interference results in a global deterioration of performance. The problem is magnified by the bandwidth-constrained and cache-constrained nature of modern computing systems.
%Despite this fact, many stat-of-the-art dynamic schedulers still follow the goal of maximizing resource usage while minimizing scheduling overheads. 
One way to avoid the problem of resource oversubscription is to spread the execution of threads over the hardware places in the system, an approach similar to OpenMP's  OMP\_PROC\_BIND=spread option~\cite{openmp45-api}. Spreading threads, however, only alleviates the problem as shared resources can still cause contention. A more aggressive approach is to aggregate enough resources (caches, cores, etc) into a task's execution place such that potentially interfering activities within the same application execute in a different place or are forced to wait~\cite{pericas-taco18}. In practice, this translates into providing each task with enough threads. %(possibly beyond their own parallelism) 
%until interference is avoided. 
However, this approach is not able to deal with inter-application interference sources such as OS jitter or co-scheduled applications. 
%In this work  current paper describes a runtime solution to address this problem. 
%Prior research suggests that mixed-mode parallel computations, in which the nodes of a computational task-DAG are themselves parallel computations that can be assigned different amounts of processing resources~\cite{pericas-taco18,chakrabarti-jpdc97,wimmer-spaa11}, are a promising execution model for modern hierarchical platforms that exhibit performance asymmetry. 
%This scheme, which we call Elastic Places~\cite{pericas-taco18}, targets interference-free scheduling for the internal tasks and allows to retain the greedy property in the global scheduler. 



% However, the greedy scheduling theorem assumes that tasks executing in parallel do not interfere with each other. It also assumes that memory bandwidth is not a limiting factor. In practice, resources such as memory bandwidth, or shared cache capacity are heavily contended, leading to slowdown and non-linear scaling of greedy scheduling. One way to address this limitation is to convert the classical 1-task to 1-core scheduling problem into a hierarchical problem in which a global level schedules M-task-groups onto N-core-places, and a local level schedules the M-tasks onto the assigned N-cores. This scheme, known as Elastic Places, targets interference-free scheduling and allows to retain the greedy property in the global scheduler~\cite{pericas-taco18}. Furthermore, this scheme maps naturally to mixed-mode parallelism when we consider each M-task-group to be a parallel computation in a mixed-mode task graph.

% The XiTAO library\footnote{\url{https://sites.google.com/site/mpericas/xitao}} is an embodiment of this concept. In XiTAO, parallel tasks are scheduled into resource partitions called Elastic Places~\cite{pericas-taco18}. The method has been shown to perform efficiently on homogeneous manycore and NUMA systems. 
%Elastic Places is implemented in a runtime library called XiTAO\footnote{\url{https://sites.google.com/site/mpericas/xitao}} and has been shown to perform efficiently on homogeneous manycore and NUMA systems. %~\cite{pericas-taco18}. %XiTAO does, however, have a few major shortcomings to achieve this goal. 
% To achieve higher power efficiency, however, it is important to make XiTAO aware of heterogeneous platforms. Furthermore, XiTAO traditionally requires the programmer to statically determine the size of the N-core-places. This property limits productivity and performance portability. 
%First, it requires the user to manually specify the amount of resources to be aggregated into a place. This is not only easy to assess, but it also depends on the particular platform. Second, XiTAO runs only on homogeneous hardware. 

In this paper, we propose a runtime technique to automatically determine an effective place for each task that is guided by a simple representation of the system's instantaneous performance. By dealing with interference as a type of dynamic performance asymmetry, we attempt to alleviate its impact. 
%resource partition sizes, i.e.~in which thread/core/socket a task should execute and how many cores (moldability) should be allocated for its execution. 
%We explore how a strict resource partitioning that can grow even beyond the intra-task parallelism can be an effective method to schedule around interference episodes. 
%and where they should be scheduled (elasticity) for mixed-mode parallel applications and thereby improve execution efficiency in the presence of interference. 
%Furthermore, we research how this knowledge can be used to leverage modern single-ISA platforms with both static and dynamic sources of performance-asymmetry.
To this end, we take a priority-aware scheduler using a fixed notion of performance asymmetry and extend it %inspired by Criticality-Aware Task Scheduling (CATS)~\cite{chronaki-ics15} and extend it 
with a performance trace table (PTT) that reflects the system's performance characteristics at runtime. Despite its simplicity, the PTT provides enough information to enable interference-aware scheduling of tasks at runtime with minimum cost. Most notably, these benefits are achieved with no static knowledge about the features of the application, the interference in the system, nor the platform's system topology. This guarantees that the approach is portable across systems. % beyond what can be easily obtained with a tool such as \texttt{hwloc}~\cite{goglin-hal16}.
%Our analysis also shows that, as a side effect, our scheduler reduces the impact on the interference source.
%a simple performance tracking table that keeps track of task execution times on a per task-type basis. 
%The tracking is furthermore categorized depending on the particular resource partition, and the size of the partition. 
%We observe that this scheme not only keeps track of efficient parallelism levels, but it also is able to infer the load of the system, which allows the scheduler to target interference-free scheduling %This allows the scheduler to consider both parallel slackness and system load in a simple and natural way, 
%without the need to statically analyze the characteristics of the task DAG that is being executed. 
%Based on the PTT, we evaluate two simple scheduling algorithms based on CATS (cite) and performance bias (cite). 
%

% To validate our proposal, we evaluate the scheme using irregular DAGs %composed of parallel subcomputations 
% and the VGG-16 neural network on both an Nvidia Jetson TX2 development board featuring an heterogeneous multicore architecture, %composed of 2 $\times$ Denver 2 Cores and 4$\times$ A57 ARMv8 cores, 
% and on an Intel Xeon Haswell platform composed of two NUMA nodes and a total of 20 cores. Our experiments focus on the benefits of criticaltity-aware and interference-free scheduling on both static and dynamic heterogeneity. Sources of heterogeneity include static platform characteristics and dynamic interference episodes, such as co-scheduling of conflicting processes. We conclude by analyzing the scalability of a VGG-16 implementation on the PTT-enabled XiTAO framework.
In summary, this paper proposes a novel scheduling technique for parallel DAGs that provides the following features:
\begin{itemize}
    \item \textbf{Elasticity and moldability}, such that it infers placement and resource container width to maximize throughput for different workload categories.
    \item \textbf{Asymmetry-awareness}, such that it reacts to static and dynamic performance asymmetry and discovers effective mappings of tasks to cores without prior knowledge of the platform and the workload. %, especially those marked with high priority. 
    \item \textbf{Interference-awareness}, which is achieved by seamlessly reducing the impact of interference arising during execution.
    %\item This results in a \textbf{performance-stable} scheduling by reducing variability across runs.
\end{itemize}

The remainder of this paper is organized as follows. 
Section~\ref{background} describes the assumptions on the execution environment that form the basis for this research. 
We present our runtime approach in Section~\ref{approach}. 
Section~\ref{setup} describes the experimental setup and benchmarks in detail, which are used to evaluate our approach in Section~\ref{Perf_Eva}.
Section~\ref{RelatedWork} describes related work, while Section~\ref{conclusion} concludes the work. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Performance asymmetry is an inherent aspect of modern computing systems~\cite{sbala-isca05}. 
% Asymmetry can be broadly attributed into two sources - static and dynamic. Static sources are fixed at design time, for example, single-ISA cores with different compute capabilities (e.g.,~big.LITTLE), or asymmetric ISA systems consisting of processor cores and accelerators (e.g.,~CPU/GPU/FPGA platforms). Dynamic sources are due to changes in resource allocated to an application (for e.g. DVFS~\cite{lesueur-hotpower10}, caches~\cite{iyer-sigmetrics07}) at runtime. 

% In modern multi-core systems the availability of shared resources (like LLC, memory bandwidth etc.)  is impacted due to interference – be it from co-running applications [refs] or the OS [refs]. Adapting to varying sources of performance asymmetry is critical to achieve efficient execution, especially for parallel applications in which inter-process synchronization can be frequent. Furthermore, the growing landscape of asymmetric system configurations complicates application scheduling since ensuring high, sustained and portable performance in such an environment is challenging. 

% Task-based parallel programming models are a natural fit in this context because they allow for tasks to be scheduled dynamically based on resource availability. Modern programming models even accommodates features like inter-task dependency specification, task priority, intra-task parallelism to help improve parallelism exploitation [ref]. Although dynamic scheduling - based on work stealing - employed by such models are better suited at adapting to asymmetry than the static scheduling counterparts there is lot of scope for improvement. This is because greedy scheduling~\cite{blumofe-jacm99}, a scheme implemented by many task-based work stealing runtime systems~\cite{contreras-iiswc11,duran-ppl11,frigo-cilk5}, always attempts to schedule a ready task as long as there are idle processing units, irrespective of whether the resulting schedule may cause interference and result in deterioration of performance. The problem is magnified by the bandwidth-constrained and cache-constrained nature of modern computing systems. 

% Recent works have attempted to improve the performance of such models by exploiting information about static performance asymmetry to efficiently schedule tasks in an asymmetric architecture [CATS]. They specifically leverage information about task priorities and schedule tasks with higher priorities on the large core in a big.LITTLE platform. Some works have attempted to study and address interference from the OS and co-running applications especially in the context of supercomputers, where application scalability is particularly impacted [refs]. Common strategies to reduce noise in this particular scenario include eliminating unnecessary activities such as process scheduling or memory management [ref] and carefully managing interrupts to minimize application perturbation [ref]. However, to our knowledge there are no proposed solutions in literature to address the diverse list of interference sources shown in Figure 1 since optimizing a system to eliminate all sources of interference is an  very challenging endeavor.

% Our proposed approach to tackle the interference accepts that interference will be present, and tries to adapt software runtimes to deal with its effects. To this end, we take a priority-aware scheduler using a fixed notion of performance asymmetry and extend it with a performance trace table (PTT) that reflects the system’s performance characteristics at runtime. Despite its simplicity, the PTT
% provides enough information to enable interference-aware scheduling of tasks at runtime with minimum cost. Most notably, these benefits are achieved with no static knowledge about the features of the application, the interference in the system, nor the platform’s system topology. This guarantees that the approach is portable across systems.


% In summary, this paper proposes a novel scheduling technique for parallel DAGs that provides the following features:
% – Elasticity and moldability, such that it infers placement and resource
% container width to maximize throughput for different workload categories.
% – Asymmetry-awareness, such that it reacts to static and dynamic perfor-
% mance asymmetry and discovers effective mappings of tasks to cores without
% prior knowledge of the platform and the workload.
% – Interference-awareness, which is achieved by seamlessly reducing the im-
% pact of interference arising during execution.

% The remainder of this paper is organized as follows. Section 2 describes the
% assumptions on the execution environment that form the basis for this research.
% We present our runtime approach in Section 3. Section 4 describes the experimen-
% tal setup and benchmarks in detail, which are used to evaluate our approach in
% Section 5. Section 6 describes related work, while Section 7 concludes the work.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
